Inference for change-plane regression

A key challenge in analyzing the behavior of change-plane estimators is that the objective function has multiple minimizers. Two estimators are proposed to deal with this non-uniqueness. For each estimator, an n-rate of convergence is established, and the limiting distribution is derived. Based on these results, we provide a parametric bootstrap procedure for inference. The validity of our theoretical results and the finite sample performance of the bootstrap are demonstrated through simulation experiments. We illustrate the proposed methods to latent subgroup identification in precision medicine using the ACTG175 AIDS study data.

==> Bernoulli_2023_Oct/cp_Sec4_cons_main_x_.tex <==
%\section{Consistency}\label{sec:con}
% \noteHC{This section is merged into the rates of convergence section.}\\
% We now establish consistency of $\hat{\theta}_n$ and $\check{\theta}_n$ in the following theorem.
% \begin{theorem}\label{thm.1}{(consistency)}
% Let $\tilde{\theta}_n$ be any sequence in $K_n^{\ast}$ satisfying $M_n(\tilde{\theta}_n)\leq M_n(\theta_0)$ for all $n$ large enough almost surely.
% Under Conditions {C1, C2, C3, C4 and C5}, $\tilde{\theta}_n\rightarrow\theta_0$ almost surely.
% \end{theorem}
% \red{That both $\hat{\theta}_n$ and $\check{\theta}_n$ are sequences satisfying the conditions of Theorem~\ref{thm.1} implies the consistency of the estimators. The proof is in Appendix \ref{asec:con} of Supplementary Material. }


